Circumventing Backdoor Defenses That Are Based on Latent Separability

Recent studies revealed that deep learning is susceptible to backdoor poisoning attacks. An adversary can embed a hidden backdoor into a model to manipulate its predictions by only modifying a few training data, without controlling the training process. Currently, a tangible signature has been widely observed across a diverse set of backdoor poisoning attacks -- models trained on a poisoned dataset tend to learn separable latent representations for poison and clean samples. This latent separation is so pervasive that a family of backdoor defenses directly take it as a default assumption (dubbed latent separability assumption), based on which to identify poison samples via cluster analysis in the latent space. An intriguing question consequently follows: is the latent separation unavoidable for backdoor poisoning attacks? This question is central to understanding whether the assumption of latent separability provides a reliable foundation for defending against backdoor poisoning attacks. In this paper, we design adaptive backdoor poisoning attacks to present counter-examples against this assumption. Our methods include two key components: (1) a set of trigger-planted samples correctly labeled to their semantic classes (other than the target class) that can regularize backdoor learning; (2) asymmetric trigger planting strategies that help to boost attack success rate (ASR) as well as to diversify latent representations of poison samples. Extensive experiments on benchmark datasets verify the effectiveness of our adaptive attacks in bypassing existing latent separation based backdoor defenses. Moreover, our attacks still maintain a high attack success rate with negligible clean accuracy drop. Our studies call for defense designers to take caution when leveraging latent separation as an assumption in their defenses.

==> assets/algorithm.tex <==
\begin{wrapfigure}{l}{0.55\textwidth}
\centering
    \begin{algorithm}[H]
    \ttfamily \small{
        \caption{Sketch of Our Adaptive Attack}\label{alg:attack_algorithm_sketch}
        \kwInput{TBD}
        \kwOutput{TBD}
        
        ~\\
        
        TBD
        
        }
    \end{algorithm}
\end{wrapfigure}

==> assets/checklist.tex <==
\section*{Checklist}


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    %\answerTODO{} 
    \answerYES. See Sec~\ref{sec:methodology}, Sec~\ref{sec:experiment}, Tab~\ref{tab:cifar10_main_results} and Tab~\ref{tab:cifar10_other_results}.
  \item Did you describe the limitations of your work?
    %\answerTODO{}
    \answerYES. See Sec~\ref{sec:discussions}
  \item Did you discuss any potential negative societal impacts of your work?
    %\answerTODO{}
    \answerYES. See Sec~\ref{sec:discussions}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    %\answerTODO{}
    \answerYES
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    %\answerTODO{}
    \answerNA~This is an empirical work.
    
    \item Did you include complete proofs of all theoretical results?
    %\answerTODO{}
    \answerNA~This is an empirical work.
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    %\answerTODO{}
    \answerYES~We provide our code in supplementary material.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    %\answerTODO{}
    \answerYES. See Appendix~\ref{appendix:experiment_configurations}
    
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
        %\answerTODO{}
        \answerNO~\textbf{But all experiments are repeated three times with different random seeds, and we report the average results.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    %\answerTODO{}
        \answerYES. See Appendix~\ref{appendix:computational_environments}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    %\answerTODO{}
    \answerYES
  \item Did you mention the license of the assets?
    %\answerTODO{}
    \answerYES.
  \item Did you include any new assets either in the supplemental material or as a URL?
    %\answerTODO{}
    \answerNA
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    %\answerTODO{}
    \answerNA
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    %\answerTODO{}
    \answerNA
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    %\answerTODO{}
    \answerNA
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    %\answerTODO{}
    \answerNA
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    %\answerTODO{}
    \answerNA
\end{enumerate}


\end{enumerate}

==> assets/naive_vs_adaptive.tex <==
\begin{figure}
\centering
\begin{subfigure}{0.18\textwidth}
\includegraphics[width=\textwidth]{fig/reps/blend.png}
    \caption{Blend~\cite{Chen2017TargetedBA}}
    \label{fig:vis_blend}
\end{subfigure}
\quad
\begin{subfigure}{0.18\textwidth}
    \includegraphics[width=\textwidth]{fig/reps/adaptive_blend.png}
    \caption{Adaptive-Blend}
    \label{fig:vis_adaptive_blend}
\end{subfigure}
\quad
\begin{subfigure}{0.18\textwidth}
\includegraphics[width=\textwidth]{fig/reps/k_triggers.png}
    \caption{K Triggers}
    \label{fig:vis_k_triggers}
\end{subfigure}
\quad
\begin{subfigure}{0.18\textwidth}
    \includegraphics[width=\textwidth]{fig/reps/adaptive_k.png}
    \caption{Adaptive-K}
    \label{fig:vis_adaptive_k}
\end{subfigure}
\caption{PCA visualization of latent separability characteristic on CIFAR-10.}
\label{fig:vis_naive_vs_adaptive}
\end{figure}


% \begin{figure}
% \centering
% \begin{subfigure}{0.35\textwidth}
% \includegraphics[width=\textwidth]{fig/compare_reps/compare_blend.png}
%     \caption{Blend~\cite{Chen2017TargetedBA}}
%     \label{fig:vis_compare_blend_2}
% \end{subfigure}
% \quad
% \begin{subfigure}{0.35\textwidth}
%     \includegraphics[width=\textwidth]{fig/compare_reps/compare_adaptive_blend.png}
%     \caption{Adaptive-Blend~(Ours)}
%     \label{fig:vis_compare_adaptive_blend_2}
% \end{subfigure}
% \\
% \begin{subfigure}{0.35\textwidth}
% \includegraphics[width=\textwidth]{fig/compare_reps/compare_k_triggers.png}
%     \caption{K Triggers}
%     \label{fig:vis_compare_k_triggers_2}
% \end{subfigure}
% \quad
% \begin{subfigure}{0.35\textwidth}
%     \includegraphics[width=\textwidth]{fig/compare_reps/compare_adaptive_k.png}
%     \caption{Adaptive-K~(Ours)}
%     \label{fig:vis_compare_adaptive_k_2}
% \end{subfigure}
% \caption{\textbf{Latent space visualized by PCA.} The left-hand plot in each subfigure corresponds to the backdoored model trained without data augmentation, while the right-hand plot corresponds to another that is trained with data augmentation.}
% \label{fig:vis_naive_vs_adaptive}
% \end{figure}

==> assets/suppressed_separability.tex <==
\begin{figure}
\centering
\begin{subfigure}{0.49\textwidth}
\includegraphics[width=\textwidth]{fig/compare_reps/compare_adaptive_blend.png}
    \caption{Adaptive-Blend~(Ours)}
    \label{fig:vis_compare_adaptive_blend}
\end{subfigure}
\hfill
\begin{subfigure}{0.49\textwidth}
    \includegraphics[width=\textwidth]{fig/compare_reps/compare_adaptive_k.png}
    \caption{Adaptive-K~(Ours)}
    \label{fig:vis_compare_adaptive_k}
\end{subfigure}
\caption{Adaptive backdoor poisoning attacks significantly reduce the latent separability between poison and clean samples. We also consider the effect of data augmentation during model training. The left-hand plot in each subfigure corresponds to the backdoored model trained without data augmentation, while the right-hand plot corresponds to another that is trained with data augmentation.}
\label{fig:vis_suppressed_separability}
\end{figure}

==> assets/visualization_latent_compare_repeat_oracle.tex <==
\begin{figure}
\centering
\begin{subfigure}{0.4\textwidth}
    \begin{tabular}{|@{}r@{}|@{}l@{}|} \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_TaCT_0.005_alpha=0.200_cover=0.005_trigger=trojan_square_32.png_poison_seed=0_full_base_no_aug_seed=666.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_TaCT_0.005_alpha=0.200_cover=0.005_trigger=trojan_square_32.png_poison_seed=0_full_base_aug_seed=666.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_TaCT_0.005_alpha=0.200_cover=0.005_trigger=trojan_square_32.png_poison_seed=0_full_base_no_aug_seed=999.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_TaCT_0.005_alpha=0.200_cover=0.005_trigger=trojan_square_32.png_poison_seed=0_full_base_aug_seed=999.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_TaCT_0.005_alpha=0.200_cover=0.005_trigger=trojan_square_32.png_poison_seed=0_full_base_no_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_TaCT_0.005_alpha=0.200_cover=0.005_trigger=trojan_square_32.png_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} \\ \hline
    \end{tabular}
    \caption{TaCT~\cite{tang2021demon}}
    \label{fig:vis_TaCT_repeat_oracle}
\end{subfigure}
\\
\begin{subfigure}{0.4\textwidth}
    \begin{tabular}{|@{}r@{}|@{}l@{}|} \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_blend_0.005_alpha=0.200_trigger=hellokitty_32.png_poison_seed=0_full_base_no_aug_seed=666.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_blend_0.005_alpha=0.200_trigger=hellokitty_32.png_poison_seed=0_full_base_aug_seed=666.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_blend_0.005_alpha=0.200_trigger=hellokitty_32.png_poison_seed=0_full_base_no_aug_seed=999.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_blend_0.005_alpha=0.200_trigger=hellokitty_32.png_poison_seed=0_full_base_aug_seed=999.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_blend_0.005_alpha=0.200_trigger=hellokitty_32.png_poison_seed=0_full_base_no_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_blend_0.005_alpha=0.200_trigger=hellokitty_32.png_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} \\ \hline
    \end{tabular}
    \caption{Blend~\cite{Chen2017TargetedBA}}
    \label{fig:vis_blend_repeat_oracle}
\end{subfigure}
\quad
\begin{subfigure}{0.4\textwidth}
    \begin{tabular}{|@{}r@{}|@{}l@{}|} \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_k_0.005_cover=0.000_poison_seed=0_full_base_no_aug_seed=666.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_k_0.005_cover=0.000_poison_seed=0_full_base_aug_seed=666.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_k_0.005_cover=0.000_poison_seed=0_full_base_no_aug_seed=999.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_k_0.005_cover=0.000_poison_seed=0_full_base_aug_seed=999.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_k_0.005_cover=0.000_poison_seed=0_full_base_no_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_k_0.005_cover=0.000_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} \\ \hline
    \end{tabular}
    \caption{K Triggers}
    \label{fig:vis_k_triggers_repeat_oracle}
\end{subfigure}
\\
\begin{subfigure}{0.4\textwidth}
    \begin{tabular}{|@{}r@{}|@{}l@{}|} \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_blend_0.005_alpha=0.200_cover=0.005_trigger=hellokitty_32.png_poison_seed=0_full_base_no_aug_seed=666.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_blend_0.005_alpha=0.200_cover=0.005_trigger=hellokitty_32.png_poison_seed=0_full_base_aug_seed=666.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_blend_0.005_alpha=0.200_cover=0.005_trigger=hellokitty_32.png_poison_seed=0_full_base_no_aug_seed=999.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_blend_0.005_alpha=0.200_cover=0.005_trigger=hellokitty_32.png_poison_seed=0_full_base_aug_seed=999.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_blend_0.005_alpha=0.200_cover=0.005_trigger=hellokitty_32.png_poison_seed=0_full_base_no_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_blend_0.005_alpha=0.200_cover=0.005_trigger=hellokitty_32.png_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} \\ \hline
    \end{tabular}
    \caption{Adaptive-Blend~(Ours)}
    \label{fig:vis_adaptive_blend_repeat_oracle}
\end{subfigure}
\quad
\begin{subfigure}{0.4\textwidth}
    \begin{tabular}{|@{}r@{}|@{}l@{}|} \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_k_0.005_cover=0.010_poison_seed=0_full_base_no_aug_seed=666.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_k_0.005_cover=0.010_poison_seed=0_full_base_aug_seed=666.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_k_0.005_cover=0.010_poison_seed=0_full_base_no_aug_seed=999.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_k_0.005_cover=0.010_poison_seed=0_full_base_aug_seed=999.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_k_0.005_cover=0.010_poison_seed=0_full_base_no_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_k_0.005_cover=0.010_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} \\ \hline
    \end{tabular}
    \caption{Adaptive-K~(Ours)}
    \label{fig:vis_adaptive_k_repeat_oracle}
\end{subfigure}

        
\caption{[Oracle] Visualization of the latent representation space~(CIFAR10). Each plot is a histogram, where the X-coordinate is the \textbf{signed} distance to the oracle hyperplane~(approximated by SVM) and Y-coordinate denotes the number of samples for the corresponding distance level. The X-coordinate range of all histograms is [-3,3] and the Y-coordinate range is [0, 75]. Bars that exceed the maximum Y range are directly cutoff at the maximum height, since the information is not important. Red bars correspond to poison samples and blue bars correspond to clean samples.}
\label{fig:vis_latent_space_compare_repeat_oracle}
\end{figure}


==> assets/visualization_latent_compare_repeat_pca.tex <==
\begin{figure}
\centering
\begin{subfigure}{0.4\textwidth}
    \begin{tabular}{|@{}r@{}|@{}l@{}|} \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_none_0.000_poison_seed=0_full_base_no_aug_seed=666.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_none_0.000_poison_seed=0_full_base_aug_seed=666.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_none_0.000_poison_seed=0_full_base_no_aug_seed=999.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_none_0.000_poison_seed=0_full_base_aug_seed=999.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_none_0.000_poison_seed=0_full_base_no_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_none_0.000_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} \\ \hline
    \end{tabular}
    \caption{No Poison}
    \label{fig:vis_none_repeat_pca}
\end{subfigure}
\quad
\begin{subfigure}{0.4\textwidth}
    \begin{tabular}{|@{}r@{}|@{}l@{}|} \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_TaCT_0.005_alpha=0.200_cover=0.005_trigger=trojan_square_32.png_poison_seed=0_full_base_no_aug_seed=666.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_TaCT_0.005_alpha=0.200_cover=0.005_trigger=trojan_square_32.png_poison_seed=0_full_base_aug_seed=666.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_TaCT_0.005_alpha=0.200_cover=0.005_trigger=trojan_square_32.png_poison_seed=0_full_base_no_aug_seed=999.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_TaCT_0.005_alpha=0.200_cover=0.005_trigger=trojan_square_32.png_poison_seed=0_full_base_aug_seed=999.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_TaCT_0.005_alpha=0.200_cover=0.005_trigger=trojan_square_32.png_poison_seed=0_full_base_no_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_TaCT_0.005_alpha=0.200_cover=0.005_trigger=trojan_square_32.png_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} \\ \hline
    \end{tabular}
    \caption{TaCT~\cite{tang2021demon}}
    \label{fig:vis_TaCT_repeat_pca}
\end{subfigure}
\\
\begin{subfigure}{0.4\textwidth}
    \begin{tabular}{|@{}r@{}|@{}l@{}|} \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_blend_0.005_alpha=0.200_trigger=hellokitty_32.png_poison_seed=0_full_base_no_aug_seed=666.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_blend_0.005_alpha=0.200_trigger=hellokitty_32.png_poison_seed=0_full_base_aug_seed=666.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_blend_0.005_alpha=0.200_trigger=hellokitty_32.png_poison_seed=0_full_base_no_aug_seed=999.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_blend_0.005_alpha=0.200_trigger=hellokitty_32.png_poison_seed=0_full_base_aug_seed=999.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_blend_0.005_alpha=0.200_trigger=hellokitty_32.png_poison_seed=0_full_base_no_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_blend_0.005_alpha=0.200_trigger=hellokitty_32.png_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} \\ \hline
    \end{tabular}
    \caption{Blend~\cite{Chen2017TargetedBA}}
    \label{fig:vis_blend_repeat_pca}
\end{subfigure}
\quad
\begin{subfigure}{0.4\textwidth}
    \begin{tabular}{|@{}r@{}|@{}l@{}|} \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_k_0.005_cover=0.000_poison_seed=0_full_base_no_aug_seed=666.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_k_0.005_cover=0.000_poison_seed=0_full_base_aug_seed=666.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_k_0.005_cover=0.000_poison_seed=0_full_base_no_aug_seed=999.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_k_0.005_cover=0.000_poison_seed=0_full_base_aug_seed=999.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_k_0.005_cover=0.000_poison_seed=0_full_base_no_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_k_0.005_cover=0.000_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} \\ \hline
    \end{tabular}
    \caption{K Triggers}
    \label{fig:vis_k_triggers_repeat_pca}
\end{subfigure}
\\
\begin{subfigure}{0.4\textwidth}
    \begin{tabular}{|@{}r@{}|@{}l@{}|} \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_blend_0.005_alpha=0.200_cover=0.005_trigger=hellokitty_32.png_poison_seed=0_full_base_no_aug_seed=666.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_blend_0.005_alpha=0.200_cover=0.005_trigger=hellokitty_32.png_poison_seed=0_full_base_aug_seed=666.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_blend_0.005_alpha=0.200_cover=0.005_trigger=hellokitty_32.png_poison_seed=0_full_base_no_aug_seed=999.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_blend_0.005_alpha=0.200_cover=0.005_trigger=hellokitty_32.png_poison_seed=0_full_base_aug_seed=999.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_blend_0.005_alpha=0.200_cover=0.005_trigger=hellokitty_32.png_poison_seed=0_full_base_no_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_blend_0.005_alpha=0.200_cover=0.005_trigger=hellokitty_32.png_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} \\ \hline
    \end{tabular}
    \caption{Adaptive-Blend~(Ours)}
    \label{fig:vis_adaptive_blend_repeat_pca}
\end{subfigure}
\quad
\begin{subfigure}{0.4\textwidth}
    \begin{tabular}{|@{}r@{}|@{}l@{}|} \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_k_0.005_cover=0.010_poison_seed=0_full_base_no_aug_seed=666.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_k_0.005_cover=0.010_poison_seed=0_full_base_aug_seed=666.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_k_0.005_cover=0.010_poison_seed=0_full_base_no_aug_seed=999.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_k_0.005_cover=0.010_poison_seed=0_full_base_aug_seed=999.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_k_0.005_cover=0.010_poison_seed=0_full_base_no_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_k_0.005_cover=0.010_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} \\ \hline
    \end{tabular}
    \caption{Adaptive-K~(Ours)}
    \label{fig:vis_adaptive_k_repeat_pca}
\end{subfigure}

        
\caption{[PCA] Visualization of the latent representation space~(CIFAR10). Red points correspond to poison samples and blue points correspond to clean samples.}
\label{fig:vis_latent_space_compare_repeat_pca}
\end{figure}


==> assets/visualization_latent_compare_repeat_tsne.tex <==
\begin{figure}
\centering
\begin{subfigure}{0.4\textwidth}
    \begin{tabular}{|@{}r@{}|@{}l@{}|} \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_none_0.000_poison_seed=0_full_base_no_aug_seed=666.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_none_0.000_poison_seed=0_full_base_aug_seed=666.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_none_0.000_poison_seed=0_full_base_no_aug_seed=999.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_none_0.000_poison_seed=0_full_base_aug_seed=999.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_none_0.000_poison_seed=0_full_base_no_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_none_0.000_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} \\ \hline
    \end{tabular}
    \caption{No Poison}
    \label{fig:vis_none_repeat_tsne}
\end{subfigure}
\quad
\begin{subfigure}{0.4\textwidth}
    \begin{tabular}{|@{}r@{}|@{}l@{}|} \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_TaCT_0.005_alpha=0.200_cover=0.005_trigger=trojan_square_32.png_poison_seed=0_full_base_no_aug_seed=666.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_TaCT_0.005_alpha=0.200_cover=0.005_trigger=trojan_square_32.png_poison_seed=0_full_base_aug_seed=666.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_TaCT_0.005_alpha=0.200_cover=0.005_trigger=trojan_square_32.png_poison_seed=0_full_base_no_aug_seed=999.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_TaCT_0.005_alpha=0.200_cover=0.005_trigger=trojan_square_32.png_poison_seed=0_full_base_aug_seed=999.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_TaCT_0.005_alpha=0.200_cover=0.005_trigger=trojan_square_32.png_poison_seed=0_full_base_no_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_TaCT_0.005_alpha=0.200_cover=0.005_trigger=trojan_square_32.png_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} \\ \hline
    \end{tabular}
    \caption{TaCT~\cite{tang2021demon}}
    \label{fig:vis_TaCT_repeat_tsne}
\end{subfigure}
\\
\begin{subfigure}{0.4\textwidth}
    \begin{tabular}{|@{}r@{}|@{}l@{}|} \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_blend_0.005_alpha=0.200_trigger=hellokitty_32.png_poison_seed=0_full_base_no_aug_seed=666.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_blend_0.005_alpha=0.200_trigger=hellokitty_32.png_poison_seed=0_full_base_aug_seed=666.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_blend_0.005_alpha=0.200_trigger=hellokitty_32.png_poison_seed=0_full_base_no_aug_seed=999.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_blend_0.005_alpha=0.200_trigger=hellokitty_32.png_poison_seed=0_full_base_aug_seed=999.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_blend_0.005_alpha=0.200_trigger=hellokitty_32.png_poison_seed=0_full_base_no_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_blend_0.005_alpha=0.200_trigger=hellokitty_32.png_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} \\ \hline
    \end{tabular}
    \caption{Blend~\cite{Chen2017TargetedBA}}
    \label{fig:vis_blend_repeat_tsne}
\end{subfigure}
\quad
\begin{subfigure}{0.4\textwidth}
    \begin{tabular}{|@{}r@{}|@{}l@{}|} \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_k_0.005_cover=0.000_poison_seed=0_full_base_no_aug_seed=666.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_k_0.005_cover=0.000_poison_seed=0_full_base_aug_seed=666.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_k_0.005_cover=0.000_poison_seed=0_full_base_no_aug_seed=999.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_k_0.005_cover=0.000_poison_seed=0_full_base_aug_seed=999.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_k_0.005_cover=0.000_poison_seed=0_full_base_no_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_k_0.005_cover=0.000_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} \\ \hline
    \end{tabular}
    \caption{K Triggers}
    \label{fig:vis_k_triggers_repeat_tsne}
\end{subfigure}
\\
\begin{subfigure}{0.4\textwidth}
    \begin{tabular}{|@{}r@{}|@{}l@{}|} \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_blend_0.005_alpha=0.200_cover=0.005_trigger=hellokitty_32.png_poison_seed=0_full_base_no_aug_seed=666.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_blend_0.005_alpha=0.200_cover=0.005_trigger=hellokitty_32.png_poison_seed=0_full_base_aug_seed=666.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_blend_0.005_alpha=0.200_cover=0.005_trigger=hellokitty_32.png_poison_seed=0_full_base_no_aug_seed=999.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_blend_0.005_alpha=0.200_cover=0.005_trigger=hellokitty_32.png_poison_seed=0_full_base_aug_seed=999.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_blend_0.005_alpha=0.200_cover=0.005_trigger=hellokitty_32.png_poison_seed=0_full_base_no_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_blend_0.005_alpha=0.200_cover=0.005_trigger=hellokitty_32.png_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} \\ \hline
    \end{tabular}
    \caption{Adaptive-Blend~(Ours)}
    \label{fig:vis_adaptive_blend_repeat_tsne}
\end{subfigure}
\quad
\begin{subfigure}{0.4\textwidth}
    \begin{tabular}{|@{}r@{}|@{}l@{}|} \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_k_0.005_cover=0.010_poison_seed=0_full_base_no_aug_seed=666.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_k_0.005_cover=0.010_poison_seed=0_full_base_aug_seed=666.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_k_0.005_cover=0.010_poison_seed=0_full_base_no_aug_seed=999.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_k_0.005_cover=0.010_poison_seed=0_full_base_aug_seed=999.pt_class=0.png} \\ \hline
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_k_0.005_cover=0.010_poison_seed=0_full_base_no_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.49\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_k_0.005_cover=0.010_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} \\ \hline
    \end{tabular}
    \caption{Adaptive-K~(Ours)}
    \label{fig:vis_adaptive_k_repeat_tsne}
\end{subfigure}

        
\caption{[t-SNE] Visualization of the latent representation space~(CIFAR10). Red points correspond to poison samples and blue points correspond to clean samples.}
\label{fig:vis_latent_space_compare_repeat_tsne}
\end{figure}


==> assets/visualization_other_archs.tex <==
\begin{table}[h]
\centering
\caption{Visualization of adaptive attacks on other network architectures in the latent representation space. The corresponding models are trained with data augmentation.}
\vspace{-0.8em}
\resizebox{0.99\linewidth}{!}{
    \begin{tabular}{c|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}}
    \toprule
    \textbf{Archs}$\rightarrow$ & 
    \multicolumn{2}{c}{VGG-16} &
    \multicolumn{2}{c}{MobileNet-V2}\cr
    \toprule
    % \cmidrule(lr){2-3} \cmidrule(lr){4-5}\cr
    \scriptsize{\textbf{Methods}\textbackslash\textbf{Attacks}} & Adap-Blend &
    Adap-Patch & Adap-Blend & Adap-Patch \cr
    \midrule
    % \adjustbox{raise=8ex}{PCA} &
    % \includegraphics[width=0.2\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_blend_0.005_alpha=0.200_cover=0.005_trigger=hellokitty_32.png_poison_seed=0_arch=vgg16_bn_full_base_aug.pt_class=0.png} &
    % \includegraphics[width=0.2\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_k_0.005_cover=0.010_poison_seed=0_arch=vgg16_bn_full_base_aug.pt_class=0.png} & 
    % \includegraphics[width=0.2\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_blend_0.005_alpha=0.200_cover=0.005_trigger=hellokitty_32.png_poison_seed=0_arch=mobilenetv2_full_base_aug.pt_class=0.png} &
    % \includegraphics[width=0.2\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_k_0.005_cover=0.010_poison_seed=0_arch=mobilenetv2_full_base_aug.pt_class=0.png}
    % \\ \hline
    \adjustbox{raise=6ex}{t-SNE} &
    \includegraphics[width=0.2\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_mask_0.003_alpha=0.150_cover=0.003_trigger=hellokitty_32.png_poison_seed=0_arch=vgg16_bn_full_base_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.2\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_k_0.003_cover=0.006_poison_seed=0_arch=vgg16_bn_full_base_aug_seed=2333.pt_class=0.png} & 
    \includegraphics[width=0.2\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_mask_0.003_alpha=0.150_cover=0.003_trigger=hellokitty_32.png_poison_seed=0_arch=mobilenetv2_class=0.png} &
    \includegraphics[width=0.2\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_k_0.003_cover=0.006_poison_seed=0_arch=mobilenetv2_full_base_aug_seed=999.pt_class=0.png}
    \\ \hline
    \adjustbox{raise=5ex}{Oracle} &
    \includegraphics[width=0.2\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_mask_0.003_alpha=0.150_cover=0.003_trigger=hellokitty_32.png_poison_seed=0_arch=vgg16_bn_class=0.png} &
    \includegraphics[width=0.2\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_k_0.003_cover=0.006_poison_seed=0_arch=vgg16_bn_full_base_aug_seed=2333.pt_class=0.png} & 
    \includegraphics[width=0.2\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_mask_0.003_alpha=0.150_cover=0.003_trigger=hellokitty_32.png_poison_seed=0_arch=mobilenetv2_class=0.png} &
    \includegraphics[width=0.2\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_k_0.003_cover=0.006_poison_seed=0_arch=mobilenetv2_full_base_aug_seed=999.pt_class=0.png}\\
    \bottomrule
    \end{tabular}
}

\label{fig:vis_other_archs}
\end{table}


==> assets/visualization_other_triggers.tex <==
\begin{table}[h]
\centering
\resizebox{0.99\linewidth}{!}{
    \begin{tabular}{c|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}}
    \toprule
    \scriptsize{\textbf{Method \textbackslash Trigger}} & \multicolumn{2}{c}{BadNet} & \multicolumn{2}{c}{Watermark} & \multicolumn{2}{c}{K Way} \cr
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
    & Naive & Adaptive & Naive & Adaptive & Naive & Adaptive \cr
    \midrule
    \adjustbox{raise=8ex}{PCA} &
    \includegraphics[width=0.3\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_0.005_alpha=1.000_cover=0.000_trigger=badnet_patch4_32.png_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.3\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_0.005_alpha=1.000_cover=0.005_trigger=badnet_patch4_32.png_poison_seed=0_full_base_aug_seed=666.pt_class=0.png} &
    
    \includegraphics[width=0.3\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_0.005_alpha=0.200_cover=0.000_trigger=watermark_white_32.png_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} & 
    \includegraphics[width=0.3\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_0.005_alpha=0.200_cover=0.005_trigger=watermark_white_32.png_poison_seed=0_full_base_aug_seed=666.pt_class=0.png} & 
    
    \includegraphics[width=0.3\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_k_way_0.005_cover=0.000_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.3\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_k_way_0.005_cover=0.010_poison_seed=0_full_base_aug_seed=666.pt_class=0.png} &
    
    \includegraphics[width=0.3\textwidth, valign=b]{fig/pca_all/pca_cifar10_dynamic_0.005_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.3\textwidth, valign=b]{fig/pca_all/pca_cifar10_adaptive_dynamic_0.005_cover=0.005_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png}
    \\ \hline
    
    \adjustbox{raise=8ex}{t-SNE} &
    \includegraphics[width=0.3\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_0.005_alpha=1.000_cover=0.000_trigger=badnet_patch4_32.png_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.3\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_0.005_alpha=1.000_cover=0.005_trigger=badnet_patch4_32.png_poison_seed=0_full_base_aug_seed=666.pt_class=0.png} &
    
    \includegraphics[width=0.3\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_0.005_alpha=0.200_cover=0.000_trigger=watermark_white_32.png_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.3\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_0.005_alpha=0.200_cover=0.005_trigger=watermark_white_32.png_poison_seed=0_full_base_aug_seed=666.pt_class=0.png} & 
    
    \includegraphics[width=0.3\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_k_way_0.005_cover=0.000_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.3\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_k_way_0.005_cover=0.010_poison_seed=0_full_base_aug_seed=666.pt_class=0.png} &
    
    \includegraphics[width=0.3\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_dynamic_0.005_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.3\textwidth, valign=b]{fig/tsne_all/tsne_cifar10_adaptive_dynamic_0.005_cover=0.005_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png}
    \\ \hline
    
    \adjustbox{raise=8ex}{Oracle} &
    
    \includegraphics[width=0.3\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_0.005_alpha=1.000_cover=0.000_trigger=badnet_patch4_32.png_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.3\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_0.005_alpha=1.000_cover=0.005_trigger=badnet_patch4_32.png_poison_seed=0_full_base_aug_seed=666.pt_class=0.png} &
    
    \includegraphics[width=0.3\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_0.005_alpha=0.200_cover=0.000_trigger=watermark_white_32.png_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} & 
    \includegraphics[width=0.3\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_0.005_alpha=0.200_cover=0.005_trigger=watermark_white_32.png_poison_seed=0_full_base_aug_seed=666.pt_class=0.png} & 
    
    \includegraphics[width=0.3\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_k_way_0.005_cover=0.000_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.3\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_k_way_0.005_cover=0.010_poison_seed=0_full_base_aug_seed=666.pt_class=0.png}
    &
    \includegraphics[width=0.3\textwidth, valign=b]{fig/svm_all/oracle_cifar10_dynamic_0.005_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png} &
    \includegraphics[width=0.3\textwidth, valign=b]{fig/svm_all/oracle_cifar10_adaptive_dynamic_0.005_cover=0.005_poison_seed=0_full_base_aug_seed=2333.pt_class=0.png}
    \\
    \bottomrule
    \end{tabular}
}
\caption{Visualization of adaptive attacks with other triggers in the latent representation space. The corresponding models are trained with data augmentation. See Fig~\ref{fig:vis_latent_space_compare_repeat_pca}, \ref{fig:vis_latent_space_compare_repeat_tsne} and \ref{fig:vis_latent_space_compare_repeat_oracle} for our plotting configurations.}
\label{fig:vis_other_triggers}
\end{table}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tab/cifar10_other_trigger_results.tex <==
\begin{table}[h]
\centering
\resizebox{0.8\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{@{}lccc@{}}
\begin{tabular}{clcccccccc}
\toprule
 & \textbf{Triggers}$\rightarrow$ & \multicolumn{2}{c}{BadNet} &
\multicolumn{2}{c}{Watermark} & \multicolumn{2}{c}{K Way} & \multicolumn{2}{c}{Dynamic} \cr
\cmidrule(lr){3-4} \cmidrule{5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
\textbf{Defenses}$\downarrow$ & & Naive & Adap & Naive & Adap & Naive & Adap & Naive & Adap \cr

\cmidrule(lr){3-10}

\multirow{2}*{\shortstack{Without Defense}}
& ASR & 100.0 & 54.6 & 89.6 & 85.4 & 96.2 & 66.4 & 98.8 & 56.8 \\
& Clean Accuracy & 91.7 & 91.7 & 91.6 & 91.8 & 90.9 & 91.3 & 91.6 & 91.7 \\
\midrule

\multirow{2}*{\shortstack{Spectral Signature~\cite{tran2018spectral}}}
& Elimination Rate & 100.0 & 15.1 & 57.6 & 43.9 & 22.4 & 23.7 & 86.8 & 67.2 \cr
& Sacrifice Rate & 7.0 & 7.5 & 7.2 & 7.3 & 7.4 & 7.4 & 7.1 & 7.2 \cr
\midrule

\multirow{2}*{\shortstack{Activation Clustering~\cite{chen2018activationclustering}}}
& Elimination Rate & 100.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 97.6 & 0.0 \cr
& Sacrifice Rate & 0.1 & 0.0 & 0.0 & 1.1 & 0.0 & 0.0 & 2.1 & 0.0 \cr
\midrule

\multirow{2}*{\shortstack{SCAn~\cite{tang2021demon}}}
& Elimination Rate & 100.0 & 36.3 & 93.2 & 0.0 & 92.0 & 0.0 & 95.2 & 98.0\cr
& Sacrifice Rate & 10.8 & 1.4 & 0.1 & 0.0 & 4.6 & 1.2 & 3.3 & 7.8 \cr
\midrule

\multirow{2}*{\shortstack{SPECTRE~\cite{hayase21a}}}
& Elimination Rate & 100.0 & 97.6 & 98.4 & 93.2 & 74.8 & 69.7 & 100.0 & 99.6 \cr
& Sacrifice Rate & 0.3 & 0.3 & 0.3 & 0.3 & 0.4 & 0.4 & 0.3 & 0.3 \cr
\midrule

\end{tabular}
} % \resizebox
\caption{
\textbf{Results of our adaptive attacks with other triggers.}}
\label{tab:cifar10_other_trigger_results}
\end{table}

==> tab/full_cifar10_main_results.tex <==
\begin{table}[ht]
\centering
\resizebox{0.99\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{@{}lccc@{}}
\begin{tabular}{clcccccc}
\toprule
 & ($\%$) & 
 \multicolumn{1}{c}{No Poison} &
\multicolumn{1}{c}{Blend~\cite{Chen2017TargetedBA}} &
\multicolumn{1}{c}{K Triggers} &
\multicolumn{1}{c}{TaCT~\cite{tang2021demon}} &
\multicolumn{1}{c}{\textbf{Adaptive-Blend (Ours)}} &
\multicolumn{1}{c}{\textbf{Adaptive-K (Ours)}}\cr
\cmidrule(lr){3-3} \cmidrule(lr){4-4}  \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8}

\multirow{2}*{\shortstack{Without Defense}}
& ASR & / & 92.3 & 100 & 97.7 & 54.9 & 93.3\\
& Clean Accuracy & 92 & 92 & 91.7 & 91.7 & 91.7 & 91.4 \\
\midrule

% \multicolumn{8}{c}{\textbf{Defenses based on Latent Separability}} \cr
% \midrule

\multirow{4}*{\shortstack{Spectral\\Signature\\ \cite{tran2018spectral}}}
& Elimination Rate & / & 74.4 & 78 & 68.8 & 70 & 9.6 \cr
& Sacrifice Rate & 15 & 7.2 & 7.1 & 7.2 & 7.2 & 7.5 \cr
& ASR & / & 81.8 & 13.6 & 95 & 25.5 & 78.9 \cr
& Clean Accuracy & 90.6 & 91.6 & 91.3 & 91.8 & 91.6 & 91.2 \cr
\midrule

\multirow{4}*{\shortstack{Activation\\Clustering\\ \cite{chen2018activationclustering}}}
& Elimination Rate & / & 98 & 76.8 & 95.6 & 0 & 48.4 \cr
& Sacrifice Rate & 12.3 & 40.7 & 35.8 & 35.9 & 0 & 37.2 \cr
& ASR & / & 2.6 & 4.9 & 34.4 & 54.9 & 90.9 \cr
& Clean Accuracy & 91.9 & 90.4 & 90.9 & 90.6 & 91.7 & 90.3 \cr
\midrule

\multirow{4}*{\shortstack{SCAn~\cite{tang2021demon}}}
& Elimination Rate & / & 92.4 & 88.4 & 0 & 0 & 0 \cr
& Sacrifice Rate & 0 & 3.6 & 3.8 & 0 & 0 & 0 \cr
& ASR & / & 13.2 & 3.1 & 97.7 & 56.3 & 93.3 \cr
& Clean Accuracy & 92 & 91.5 & 91.7 & 91.7 & 91.6 & 91.4 \cr
\midrule

\multirow{4}*{\shortstack{SPECTRE~\cite{hayase21a}}}
& Elimination Rate & / & 97.6 & 99.2 & 100 & 94 & 67.6 \cr
& Sacrifice Rate & 1.5 & 0.3 & 0.3 & 0.3 & 0.3 & 0.4 \cr
& ASR & / & 3.6 & 3.4 & 1.2 & 2.7 & 17.3 \cr
& Clean Accuracy & 91.8 & 92.2 & 92.2 & 91.8 & 92 & 91.4 \cr
\midrule

\end{tabular}
} % \resizebox
\caption{
\textbf{Latent separability based defenses against our adaptive attacks on CIFAR-10.}~(seed $\#1$)}
\label{tab:full_cifar10_main_results_666}
\end{table}





\begin{table}[ht]
\centering
\resizebox{0.99\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{@{}lccc@{}}
\begin{tabular}{clcccccc}
\toprule
 & ($\%$) & 
 \multicolumn{1}{c}{No Poison} &
\multicolumn{1}{c}{Blend~\cite{Chen2017TargetedBA}} &
\multicolumn{1}{c}{K Triggers} &
\multicolumn{1}{c}{TaCT~\cite{tang2021demon}} &
\multicolumn{1}{c}{\textbf{Adaptive-Blend (Ours)}} &
\multicolumn{1}{c}{\textbf{Adaptive-K (Ours)}}\cr
\cmidrule(lr){3-3} \cmidrule(lr){4-4}  \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8}

\multirow{2}*{\shortstack{Without Defense}}
& ASR & / & 91.2 & 100.0 & 98.5 & 54.7 & 99.6  \\
& Clean Accuracy & 92.1 & 91.8 & 91.9 & 91.8 & 91.6 & 91.7 \\
\midrule

% \multicolumn{8}{c}{\textbf{Defenses based on Latent Separability}} \cr
% \midrule

\multirow{4}*{\shortstack{Spectral\\Signature\\ \cite{tran2018spectral}}}
& Elimination Rate & / & 48.0 & 84.4 & 82.0 & 56.8 & 12.8 \cr
& Sacrifice Rate & 15.0 & 7.3 & 7.1 & 7.1 & 7.3 & 7.5 \cr
& ASR & / & 91.0 & 7.8 & 93.9 & 32.0 & 98.7 \cr
& Clean Accuracy & 90.8 & 91.7 & 91.5 & 91.2 & 91.7 & 91.4 \cr
\midrule

\multirow{4}*{\shortstack{Activation\\Clustering\\ \cite{chen2018activationclustering}}}
& Elimination Rate & / & 82.8 & 90.4 & 100.0 & 0.0 & 42.0  \cr
& Sacrifice Rate & 12.3 & 36.5 & 36.2 & 36.0 & 0.0 & 37.2 \cr
& ASR & / & 67.2 & 3.3 & 0.6 & 54.7 & 97.7 \cr
& Clean Accuracy & 91.6 & 91.0 & 90.4 & 90.6 & 91.6 & 90.1 \cr
\midrule

\multirow{4}*{\shortstack{SCAn~\cite{tang2021demon}}}
& Elimination Rate & / & 90.4 & 91.6 & 100.0 & 0.0 & 2.8 \cr
& Sacrifice Rate & 0.0 & 0.1 & 3.6 & 3.3 & 0.0 & 9.4 \cr
& ASR & / & 16.3 & 3.8 & 0.7 & 54.7 & 99.1 \cr
& Clean Accuracy & 92.1 & 91.8 & 91.8 & 91.2 & 91.6 & 88.4 \cr
\midrule

\multirow{4}*{\shortstack{SPECTRE~\cite{hayase21a}}}
& Elimination Rate & / & 96.0 & 99.2 & 100.0 & 94.8 & 0.0 \cr
& Sacrifice Rate & 1.5 & 0.3 & 0.3 & 0.3 & 0.3 & 8.0 \cr
& ASR & / & 10.3 & 1.6 & 1.5 & 2.3 & 98.0 \cr
& Clean Accuracy & 91.4 & 91.8 & 91.9 & 91.5 & 91.3 & 91.1 \cr
\midrule

\end{tabular}
} % \resizebox
\caption{
\textbf{Latent separability based defenses against our adaptive attacks on CIFAR-10.}~(seed $\#2$)}
\label{tab:full_cifar10_main_results_999}
\end{table}







\begin{table}[ht]
\centering
\resizebox{0.99\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{@{}lccc@{}}
\begin{tabular}{clcccccc}
\toprule
 & ($\%$) & 
 \multicolumn{1}{c}{No Poison} &
\multicolumn{1}{c}{Blend~\cite{Chen2017TargetedBA}} &
\multicolumn{1}{c}{K Triggers} &
\multicolumn{1}{c}{TaCT~\cite{tang2021demon}} &
\multicolumn{1}{c}{\textbf{Adaptive-Blend (Ours)}} &
\multicolumn{1}{c}{\textbf{Adaptive-K (Ours)}}\cr
\cmidrule(lr){3-3} \cmidrule(lr){4-4}  \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8}

\multirow{2}*{\shortstack{Without Defense}}
& ASR & / & 93.3 & 100.0 & 97.3 & 52.1 & 99.0 \\
& Clean Accuracy & 91.9 & 91.3 & 91.7 & 91.8 & 91.8 & 91.7 \\
\midrule

% \multicolumn{8}{c}{\textbf{Defenses based on Latent Separability}} \cr
% \midrule

\multirow{4}*{\shortstack{Spectral\\Signature\\ \cite{tran2018spectral}}}
& Elimination Rate & / & 62.4 & 86.8 & 80.8 & 57.2 & 11.6 \cr
& Sacrifice Rate & 15.0 & 7.2 & 7.1 & 7.1 & 7.3 & 7.5 \cr
& ASR & / & 89.8 & 7.2 & 93.6 & 32.0 & 98.7 \cr
& Clean Accuracy & 91.3 & 91.5 & 91.3 & 91.5 & 91.2 & 90.9 \cr
\midrule

\multirow{4}*{\shortstack{Activation\\Clustering\\ \cite{chen2018activationclustering}}}
& Elimination Rate & / & 96.0 & 92.8 & 100.0 & 0.0 & 38.8 \cr
& Sacrifice Rate & 12.3 & 41.6 & 41.1 & 37.6 & 0.0 & 36.5 \cr
& ASR & / & 6.9 & 2.5 & 0.5 & 52.3 & 97.7 \cr
& Clean Accuracy & 91.9 & 90.0 & 90.5 & 89.6 & 91.9 & 90.7 \cr
\midrule

\multirow{4}*{\shortstack{SCAn~\cite{tang2021demon}}}
& Elimination Rate & / & 97.2 & 89.6 & 100.0 & 0.0 & 0.0 \cr
& Sacrifice Rate & 0.0 & 2.1 & 0.0 & 0.0 & 0.0 & 0.0 \cr
& ASR & / & 2.4 & 5.5 & 1.2 & 52.1 & 99.0 \cr
& Clean Accuracy & 91.9 & 92.0 & 91.9 & 91.9 & 91.8 & 91.7 \cr
\midrule

\multirow{4}*{\shortstack{SPECTRE~\cite{hayase21a}}}
& Elimination Rate & / & 95.2 & 99.2 & 100.0 & 96.4 & 0.0 \cr
& Sacrifice Rate & 1.5 & 0.3 & 0.3 & 0.3 & 0.3 & 0.8 \cr
& ASR & / & 10.9 & 3.9 & 0.4 & 3.1 & 99.5 \cr
& Clean Accuracy & 91.6 & 91.8 & 91.5 & 91.7 & 92.1 & 91.5 \cr
\midrule

\end{tabular}
} % \resizebox
\caption{
\textbf{Latent separability based defenses against our adaptive attacks on CIFAR-10.}~(seed $\#3$)}
\label{tab:full_cifar10_main_results_2333}
\end{table}



==> tab/full_cifar10_other_results.tex <==
\begin{table}[ht]
\centering
\resizebox{0.99\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{@{}lccc@{}}
\begin{tabular}{ccccccccccccccc}
\toprule
\textbf{Defenses$\rightarrow$} &
\multicolumn{2}{c}{FP~\cite{liu2018fine}} &
\multicolumn{4}{c}{STRIP (C)~\cite{gao2019strip}} & 
\multicolumn{2}{c}{STRIP (F)~\cite{gao2019strip}} & 
\multicolumn{3}{c}{NC}~\cite{wang2019neural} & 
\multicolumn{3}{c}{ABL~\cite{li2021anti}} \cr
\cmidrule(lr){2-3} \cmidrule(lr){4-7} \cmidrule(lr){8-9} \cmidrule(lr){10-12} \cmidrule(lr){13-15}
\textbf{Attacks} $\downarrow$ & ASR & CA & Eli & Sac & ASR & CA & Eli & Sac & AI & ASR & CA & IP & ASR & CA \cr
\midrule
Adaptive-Blend & 61.9 & 81.1 & 1.6 & 10.4 & 52.1 & 91.4 & 1.1 & 10.0 & 3.7 & 27.4 & 89.3 & 0.0 & 41.7 & 80.3 \cr
\midrule
Adaptive-K & 68.2 & 80.3 & 5.6 & 10.6 & 91.5 & 91.3 & 100.0 & 10.0 & 3.6 & 1.9 & 90.7 & 1.0 & 96.3 & 91.0\cr
\bottomrule

\end{tabular}
} % \resizebox
\caption{
\textbf{Other defenses against our adaptive attacks on CIFAR-10.}~(seed $\#1$)}
\label{tab:full_cifar10_other_results_666}
\end{table}



\begin{table}[ht]
\centering
\resizebox{0.99\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{@{}lccc@{}}
\begin{tabular}{ccccccccccccccc}
\toprule
\textbf{Defenses$\rightarrow$} &
\multicolumn{2}{c}{FP~\cite{liu2018fine}} &
\multicolumn{4}{c}{STRIP (C)~\cite{gao2019strip}} & 
\multicolumn{2}{c}{STRIP (F)~\cite{gao2019strip}} & 
\multicolumn{3}{c}{NC}~\cite{wang2019neural} & 
\multicolumn{3}{c}{ABL~\cite{li2021anti}} \cr
\cmidrule(lr){2-3} \cmidrule(lr){4-7} \cmidrule(lr){8-9} \cmidrule(lr){10-12} \cmidrule(lr){13-15}
\textbf{Attacks} $\downarrow$ & ASR & CA & Eli & Sac & ASR & CA & Eli & Sac & AI & ASR & CA & IP & ASR & CA \cr
\midrule
Adaptive-Blend & 20.9 & 79.7 & 0.8 & 9.8 & 56.3 & 91.4 & 1.1 & 10.0 & 0.6 & 48.8 & 89.9 & 0.0 & 48.5 & 85.1 \cr
\midrule
Adaptive-K & 85.3 & 77.2 & 14.0 & 10.1 & 99.7 & 90.8 & 100.0 & 10.0 & 2.8 & 3.9 & 90.5 & 0.8 & 96.2 & 91.0 \cr
\bottomrule

\end{tabular}
} % \resizebox
\caption{
\textbf{Other defenses against our adaptive attacks on CIFAR-10.}~(seed $\#2$)}
\label{tab:full_cifar10_other_results_999}
\end{table}



\begin{table}[ht]
\centering
\resizebox{0.99\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{@{}lccc@{}}
\begin{tabular}{ccccccccccccccc}
\toprule
\textbf{Defenses$\rightarrow$} &
\multicolumn{2}{c}{FP~\cite{liu2018fine}} &
\multicolumn{4}{c}{STRIP (C)~\cite{gao2019strip}} & 
\multicolumn{2}{c}{STRIP (F)~\cite{gao2019strip}} & 
\multicolumn{3}{c}{NC}~\cite{wang2019neural} & 
\multicolumn{3}{c}{ABL~\cite{li2021anti}} \cr
\cmidrule(lr){2-3} \cmidrule(lr){4-7} \cmidrule(lr){8-9} \cmidrule(lr){10-12} \cmidrule(lr){13-15}
\textbf{Attacks} $\downarrow$ & ASR & CA & Eli & Sac & ASR & CA & Eli & Sac & AI & ASR & CA & IP & ASR & CA \cr
\midrule
Adaptive-Blend & 61.5 & 81.6 & 0.8 & 10.6 & 56.6 & 91.3 & 1.3 & 10.0 & 0.2 & 1.3 & 89.6 & 0.0 & 34.8 & 82.7 \cr
\midrule
Adaptive-K & 63.3 & 80.5 & 10.4 & 10.7 & 99.3 & 91.3 & 100.0 & 10.0 & 4.8 & 1.6 & 90.9 & 0.8 & 96.3 & 86.3 \cr
\bottomrule

\end{tabular}
} % \resizebox
\caption{
\textbf{Other defenses against our adaptive attacks on CIFAR-10.}~(seed $\#3$)}
\label{tab:full_cifar10_other_results_2333}
\end{table}


==> tab/wanet_and_refool.tex <==
\begin{table}[ht]
\centering
\caption{Results of WaNet and Refool.}
\vspace{-0.8em}
\resizebox{0.99\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{@{}lccc@{}}
\begin{tabular}{ccccccccccccccc}
\toprule
\textbf{Defenses$\rightarrow$} &
\multicolumn{2}{c}{No Defense} &
\multicolumn{2}{c}{Spectral Signature} &
\multicolumn{2}{c}{Activation Clustering} & 
\multicolumn{2}{c}{SCAn} & 
\multicolumn{2}{c}{SPECTRE} \cr
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
\textbf{Attacks} $\downarrow$ & ASR & CA & Elimination & Sacrifice & Elimination & Sacrifice & Elimination & Sacrifice & Elimination & Sacrifice \cr
\midrule
WaNet & 26.0 & 89.9 & 47.3 & 50.3 & 0.0 & 3.4 & 93.3 & 3.2 & 54.8 & 4.4 \cr
\midrule
Refool & 57.1 & 90.0 & 75.8 & 48.6 & 84.8 & 0.1 & 83.7 & 0.1 & 74.8 & 3.6 \cr
\bottomrule

\end{tabular}
} % \resizebox
\label{tab:wanet_and_refool}
\end{table}
